Weighted Diversified Sampling for Efficient Data-Driven Single-Cell Gene-Gene Interaction Discovery

Gene-gene interactions play a crucial role in the manifestation of complex human diseases. Uncovering significant gene-gene interactions is a challenging task. Here, we present an innovative approach utilizing data-driven computational tools, leveraging an advanced Transformer model, to unearth noteworthy gene-gene interactions. Despite the efficacy of Transformer models, their parameter intensity presents a bottleneck in data ingestion, hindering data efficiency. To mitigate this, we introduce a novel weighted diversified sampling algorithm. This algorithm computes the diversity score of each data sample in just two passes of the dataset, facilitating efficient subset generation for interaction discovery. Our extensive experimentation demonstrates that by sampling a mere 1\% of the single-cell dataset, we achieve performance comparable to that of utilizing the entire dataset.

==> acknowledge.tex <==
\section{Acknowledgement}

Rongbin Li is supported by NLM Training Program in Biomedical Informatics \& Data Science for Predoctoral \& Postdoctoral Fellows under the Gulf Coast Consortia grant 5T15LM007093-31. This work is also partly supported by the National Institutes of Health (NIH) through grants 1UL1TR003167, 1UM1TR004906-01, 1R01AG066749, 1U24MH130988-01, 5R56AG069880-02, Department of Defense W81XWH-22-1-0164, and the Cancer Prevention and Research Institute of Texas through grant RP170668 (WJZ).

==> limitation.tex <==
\section{Limitations \& Broader Impact}

While the Weighted Diversified Sampling (WDS) method markedly improves the scalability of our transformer-based computational framework, the existing implementation does not permit scaling the transformer model to the level of a trillion parameters on a limited number of GPUs. Future work may involve adapting our computational framework to accommodate larger models using more substantial GPU resources. We also acknowledge the potential carbon release of GPU usage.
